Unconditionally Secure Commitments with Quantum Auxiliary Inputs

We show the following unconditional results on quantum commitments in two related yet different models: 1. We revisit the notion of quantum auxiliary-input commitments introduced by Chailloux, Kerenidis, and Rosgen (Comput. Complex. 2016) where both the committer and receiver take the same quantum state, which is determined by the security parameter, as quantum auxiliary inputs. We show that computationally-hiding and statistically-binding quantum auxiliary-input commitments exist unconditionally, i.e., without relying on any unproven assumption, while Chailloux et al. assumed a complexity-theoretic assumption, ${\bf QIP}\not\subseteq{\bf QMA}$. On the other hand, we observe that achieving both statistical hiding and statistical binding at the same time is impossible even in the quantum auxiliary-input setting. To the best of our knowledge, this is the first example of unconditionally proving computational security of any form of (classical or quantum) commitments for which statistical security is impossible. As intermediate steps toward our construction, we introduce and unconditionally construct post-quantum sparse pseudorandom distributions and quantum auxiliary-input EFI pairs which may be of independent interest. 2. We introduce a new model which we call the common reference quantum state (CRQS) model where both the committer and receiver take the same quantum state that is randomly sampled by an efficient setup algorithm. We unconditionally prove that there exist statistically hiding and statistically binding commitments in the CRQS model, circumventing the impossibility in the plain model. We also discuss their applications to zero-knowledge proofs, oblivious transfers, and multi-party computations.

==> MPC.tex <==
\section{Oblivious Transfer and MPC in the CRQS model}
We show that we can use our commitment scheme constructed in \Cref{sec:com} to construct oblivious transfer and MPC protocols for general classical and quantum functionality. 
In the plain model (where there is no CRQS), Bartusek, Coladangelo, Khurana, and Ma \cite{C:BCKM20b}
By plugging our commitments into BCKM20, we obtain OT in the CRQS model. 
Moreover, by the IPS compiler, we obtain MPC. 
Here, we have to be careful that the adversary againsnt $n$-party computation may obtain at most $n$ copies of the CRQS and thus we need to use $t$-copy secure commitments/OT for $t\geq n$. 
\begin{theorem}
There exists MPC in the CRQS model. 
\end{theorem}

==> nogo_CRS.tex <==
\section{No-go in the classical CRS model}
\label{sec:nogo_CRS}

Here we show that the impossibility of statistically-secure quantum bit commitments
holds even in the classical common reference string (CRS) model where a common classical bit string sampled from a certain distribution is
given to the committer and the receiver.
Without loss of generality,
we have only to consider
the following canonical form~\cite{AC:Yan22}. 
\begin{itemize}
    \item 
    {\bf Setup phase:}
    $\setup$ takes $1^\secp$ as input, samples $k\in\bit^\secp$ from a distribution $D_\secp$, and sends $k$ to $C$ and $R$.  
    \item
{\bf Commit phase:} 
$C$ takes $k$ given by the setup algorithm and a bit $b\in \bit$ to commit as input, generates a quantum state $\ket{\Psi_{k,b}}_{\qreg{C},\qreg{R}}$ on registers $\qreg{C}$ and $\qreg{R}$, and 
sends the register $\qreg{C}$ to $R$. 
\item
{\bf Reveal phase:}
$C$ sends $b$ and the register $\qreg{R}$ to $R$.
If the state over $\qreg{C}$ and $\qreg{R}$ is $\ket{\Psi_{k,b}}$ $R$ outputs $b$. Otherwise, it outputs $\bot$. 
\end{itemize}

Now we show that such a scheme cannot be both statistically-hiding and statistically-binding at the same time.
If the commit phase is honestly executed,
the state possessed by $R$ after the commit phase is
\begin{align}
\sum_k p_k \ket{k}\bra{k}\otimes \rho_{k,b},    
\end{align}
where $p_k$ is the probability that $k$ is sampled from $D_\secp$, and $\rho_{k,b}\coloneqq \Tr_{\qreg{R}}(\ket{\Psi_{k,b}}_{\qreg{R},\qreg{C}})$.
Let us consider the following adversary $\cA$ for hiding:
\begin{enumerate}
    \item Measure the first register in the computational basis to get $k$. 
    \item 
    Apply a certain POVM measurement $\{\Pi_k,I-\Pi_k\}$ on the second register, and output 0 if $\Pi_k$ is obtained.
    Output 1 if the other one is obtained.
\end{enumerate}
Then due to the hiding,
\begin{align}
\negl(\secp)&\ge|\Pr[0\gets\cA:b=0]
-\Pr[0\gets\cA:b=1]|\\
&=\left|\sum_k p_k \Tr(\Pi_k \rho_{k,0})    
-\sum_k p_k \Tr(\Pi_k \rho_{k,1})\right|    \\
&=\left|\sum_k p_k 
[\Tr(\Pi_k \rho_{k,0})    
- \Tr(\Pi_k \rho_{k,1})]\right|    \\
&=\left|\sum_k p_k 
\|\rho_{k,0}-\rho_{k,1}\|_{\rm tr}\right|    \\
&=\sum_k p_k 
\|\rho_{k,0}-\rho_{k,1}\|_{\rm tr}    \\
&\ge\sum_k p_k 
(1-F(\rho_{k,0},\rho_{k,1})),
\end{align}
where each $\Pi_k$ is chosen such that 
$\Tr(\Pi_k\rho_{k,0})-\Tr(\Pi_k\rho_{k,1})=\|\rho_{k,0}-\rho_{k,1}\|_{\rm tr}$.
This means
\begin{align}
\sum_k p_k F(\rho_{k,0},\rho_{k,1})\ge1-\negl(\secp).
\end{align}
Let us consider the following adversary $\cB$ that breaks hiding as follows:
\begin{enumerate}
\item 
Get $k$ as input.
    \item 
    Honestly commit $b=0$.
    \item 
    Apply a certain unitary $U^k$ on $\qreg{R}$ and send it to $R$.
\end{enumerate}
The probability that $R$ outputs $b=1$ is
\begin{align}
   \sum_k p_k |\bra{\Psi_{k,1}}(I_{\qreg{C}}\otimes U^k_{\qreg{R}})\ket{\Psi_{k,0}} |^2
   &=
   \sum_k p_k
   F(\rho_{k,0},\rho_{k,1})\\
   &\ge1-\negl(\secp),
\end{align}
where each $U^k$ is taken such that $F(\rho_{k,0},\rho_{k,1})=|\bra{\Psi_{k,1}}(I_{\qreg{C}}\otimes U_{\qreg{R}}^k)\ket{\Psi_{k,0}}|^2$.
Therefore $\cB$ breaks the binding.

